What is Learned in Visually Grounded Neural Syntax Acquisition

Visual features are a promising signal for learning bootstrap textual models. However, blackbox learning models make it difficult to isolate the specific contribution of visual components. In this analysis, we consider the case study of the Visually Grounded Neural Syntax Learner (Shi et al., 2019), a recent approach for learning syntax from a visual training signal. By constructing simplified versions of the model, we isolate the core factors that yield the model's strong performance. Contrary to what the model might be capable of learning, we find significantly less expressive versions produce similar predictions and perform just as well, or even better. We also find that a simple lexical signal of noun concreteness plays the main role in the model's predictions as opposed to more complex syntactic reasoning.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> sup-datamodels.tex <==


For our main experiments, we follow \citet{Shi2019:vgsnl} and train all the \vgnsl variations on 82,783 images and 413,915 captions from the MSCOCO training set. We  evaluate the unsupervised constituency paser performance  using 5,000 non-overlapping test captions. We generate binary gold-trees using Benepar~\citep{Kitaev:18benepar}, an off-the-shelf supervised constituency parser.

We use additional 5,000 non-overlapping development captions for our analyses and visualization in Section~\ref{sec:exp}.
We analyze our simplified variations of \vgnsl trained with the best performing training configuration +HI+FastText-IN.



